BoMuDANet: Unsupervised Adaptation for Visual Scene Understanding in Unstructured Driving Environments

We present an unsupervised adaptation approach for visual scene understanding in unstructured traffic environments. Our method is designed for unstructured real-world scenarios with dense and heterogeneous traffic consisting of cars, trucks, two-and three-wheelers, and pedestrians. We describe a new semantic segmentation technique based on unsupervised domain adaptation (DA), that can identify the class or category of each region in RGB images or videos. We also present a novel self-training algorithm (Alt-Inc) for multi-source DA that improves the accuracy. Our overall approach is a deep learning-based technique and consists of an unsupervised neural network that achieves 87.18% accuracy on the challenging India Driving Dataset. Our method works well on roads that may not be well-marked or may include dirt, unidentifiable debris, potholes, etc. A key aspect of our approach is that it can also identify objects that are encountered by the model for the fist time during the testing phase. We compare our method against the state-of-the-art methods and show an improvement of 5.17% - 42.9%. Furthermore, we also conduct user studies that qualitatively validate the improvements in visual scene understanding of unstructured driving environments.

==> Tables/altInc-idd-cs-gta-bdd-adaptsegnet.tex <==
\begin{table}[t]
% \footnotesize
\centering
\caption{Iteration-wise results: Alt-Inc algorithm on the closed-set multi-source adaptation of CS, GTA, BDD to IDD} 
\divya{Replace these numbers with the corresponding ADVENT experiment once training is done} 
\label{tab:altinc}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c c c}
\hline
Iteration & Model 1 mIoU & Model 2 mIoU  \\ \\
\hline
Iteration 0 & - & 36.73 \\
Iteration 1 & 36.94 & 38.42 \\
Iteration 2 & 37.26 & 39.06 \\
Iteration 3 & 37.5 & 39.2 \\
\hline

\end{tabular}
}
\end{table}


==> Tables/datasets.tex <==
\begin{table}[t]
% \footnotesize
\centering
% \begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l c r}
\toprule
Dataset Name & Used as & Reference \\
\toprule
GTA5 & Source (Tab.\ref{tab:open_set},~\ref{tab:idd_mainresults},\ref{tab:sota}) & \cite{gta}\\
CityScapes (CS) & Source (Tab.\ref{tab:open_set},~\ref{tab:idd_mainresults},\ref{tab:sota}), Target (Tab.~\ref{tab:sota}) & \cite{cs}\\
Synscapes (SC) & Source (Tab.\ref{tab:open_set},~\ref{tab:idd_mainresults},\ref{tab:sota}) & \cite{wrenninge2018synscapes}\\
India Driving Dataset (IDD) & Source \& Target (Tab.\ref{tab:open_set},~\ref{tab:idd_mainresults},\ref{tab:sota}) & \cite{varma2019idd}\\
Berkeley Deep Drive (BDD) & Source (Tab.\ref{tab:open_set},~\ref{tab:idd_mainresults},\ref{tab:sota}) & \cite{yu2020bdd100k} \\


\bottomrule
\end{tabular}
}
\caption{\textbf{List of Datasets} (Sorted chronologically): The second column identifies the type of the domain in which that dataset is used and specifies the locations for the results on that particular domain type. For example, results on the CS dataset as a \textit{source} domain are located in Tables~\ref{tab:idd_mainresults},\ref{tab:sota}, and~\ref{tab:open_set}, while the results on the CS dataset as a \textit{target} domain are located in Table~\ref{tab:sota} only. }

\label{tab: datasets}
% \vspace{-10pt}
% \end{center}
\end{table}




==> Tables/kl_pseudo.tex <==
\begin{table}
% \footnotesize
\centering
\caption{Ablation studies on tuning the KL divergence and pseudo labels weight hyperparameter on model 1 for case (i) in Table 2 of main paper}
% \begin{center}
% \resizebox{.8\columnwidth}{!}{
\begin{tabular}{c c c}
\toprule
KL weight & Pseudo labels weight & mIoU \\
\midrule
0.0 & 1.0 & 36.63\\
0.1 & 1.0 & 36.97 \\
0.1 & 0.1 & 37.66\\
0.5 & 0.1 & 36.99\\
1.0 & 1.0 & 36.9\\
\bottomrule
\end{tabular}
% }
\label{tab:kl_pseudo}
% \end{center}
\end{table}



